Switch Points of Bi-Persistence Matching Distance

In multi-parameter persistence, the matching distance is defined as the supremum of weighted bottleneck distances on the barcodes given by the restriction of persistence modules to lines with a positive slope. In the case of finitely presented bi-persistence modules, all the available methods to compute the matching distance are based on restricting the computation to lines through pairs from a finite set of points in the plane. Some of these points are determined by the filtration data as they are entrance values of critical simplices. However, these critical values alone are not sufficient for the matching distance computation and it is necessary to add so-called switch points, i.e. points such that on a line through any of them, the bottleneck matching switches the matched pair. This paper is devoted to the algorithmic computation of the set of switch points given a set of critical values. We find conditions under which a candidate switch point is erroneous or superfluous. The obtained conditions are turned into algorithms that have been implemented. With this, we analyze how the size of the set of switch points increases as the number of critical values increases, and how it varies depending on the distribution of critical values. Experiments are carried out on various types of bi-persistence modules.

==> figures/Omega2.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (5,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
%\coordinate (c5) at ($(c2)+ (0,2)$);
  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
 \coordinate (L) at ($(3.5,0)-(40:1)$);
  \coordinate (LL) at ($(L)+(40:13)$); 
  

  \coordinate (L') at ($(3.5,0)-(55:1)$);
  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
 % \node[anchor=north] at (c1) { $c_1$};
   \draw[red, fill=red] (c2) circle (5pt);
  %\node[anchor=north] at (c2) { $c_2$};
  %\draw[black, fill=black] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
%  \node[anchor=north] at (c4) { $c_4$};
  
%\draw[dashed ](c1) -- (C);
%\draw[dashed ](c1) -- (D);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
\draw[orange, thick]  (L)--(LL);
\node[anchor=north west ] at (LL) { \color{orange}$L$};


\draw[orange, thick]  (L')--(LL');
\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> figures/Omega3.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (5,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
\coordinate (c5) at ($(c2)+ (0,2)$);
  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
 \coordinate (L) at ($(3.5,0)-(40:1)$);
  \coordinate (LL) at ($(L)+(40:13)$); 
  

  \coordinate (L') at ($(3.5,0)-(55:1)$);
  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
 % \node[anchor=north] at (c1) { $c_1$};
   \draw[red, fill=red] (c2) circle (5pt);
  %\node[anchor=north] at (c2) { $c_2$};
  %\draw[blue, fill=blue] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
%  \node[anchor=north] at (c4) { $c_4$};
\draw[green, fill=green] (c5) circle (5pt);
\node[anchor=north] at (c5) { $\omega$}; 
  
%\draw[dashed ](c1) -- (C);
%\draw[dashed ](c1) -- (D);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
\draw[orange, thick]  (L)--(LL);
\node[anchor=north west ] at (LL) { \color{orange}$L$};


\draw[orange, thick]  (L')--(LL');
\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> figures/Omega4.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (7,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
\coordinate (c5) at ($(c2)+ (0,2)$);
\coordinate (e) at ($(c1)+ (2.5,2)$);
\coordinate (f) at ($(e)+(8,0)$); 
\coordinate (g) at ($(c2)+(0,6)$);  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
% \coordinate (L) at ($(3.5,0)-(40:1)$);
%  \coordinate (LL) at ($(L)+(40:13)$); 
%  
%
%  \coordinate (L') at ($(3.5,0)-(55:1)$);
%  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
  \node[anchor=north] at (c1) { $a$};
   \draw[red, fill=red] (c2) circle (5pt);
  \node[anchor=north] at (c2) { $b$};
  %\draw[blue, fill=blue] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
  \node[anchor=north] at (c4) { $c$};
\draw[green, fill=green] (c5) circle (5pt);
\node[anchor=north] at (c5) { $\omega$}; 
\draw[black, fill=black] (e) circle (5pt);
\node[anchor=north] at (e) { $e$}; 
 
\draw[dashed ](c1) -- (c4);
\draw[dashed ](e) -- (f);
\draw[dashed ](c2) -- (g);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
%\draw[orange, thick]  (L)--(LL);
%\node[anchor=north west ] at (LL) { \color{orange}$L$};


%\draw[orange, thick]  (L')--(LL');
%\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> figures/xPushUpConvexHullNonExample.tex <==
\begin{scope}[scale =0.5]


% \coordinate (oo) at (0,0);
 %\coordinate (ox) at (10,0); 
 %\coordinate (oy) at (0, 10); 

 %points u,v,w,x
 \coordinate (u) at (1,2);
 \coordinate (w) at ($(u)+ (4,4)$); 
 \coordinate (v) at (6,0);
 \coordinate (x) at (2,0.5);

%draw points
\draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v$};
  \draw[blue, fill=blue] (x) circle (5pt);
 \node[anchor=north] at (x) { $x$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};

 %convex hull 
 \draw[fill=red!10] (u) -- (v) -- (w) -- cycle;


 
 \end{scope}


==> matching_distance/Positive_cone.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (9,0); 
 \coordinate (oy) at (0, 9); 
 \coordinate (u) at (3,3);
 \coordinate (uy) at ($(u) + (5,0)$);
 \coordinate (ux) at ($(u) + (0,5)$);
 \coordinate (nn) at (8,8); 
 
 
 % axes 
  \draw[->, ultra thick](oo) -- (ox) ;
  \draw[->, ultra thick ](oo) --(oy); 


 % u
  
  \node[anchor=north ] at (u) { $u = S_{\{1,2\}}$};
 \draw[ blue](u) -- (ux) ;
  \draw[green ](u) -- (uy) ;
  \node[anchor= north] at (uy) {$ S_{\{2\}}$};
    \node[anchor= east] at (ux) {$ S_{\{1\}}$};
  
  % pusitive cone 
\fill [fill = gray, fill opacity=0.2] (u) rectangle (nn);
 \node[anchor=north east] at (nn) { $S_+(u)$};
 
 \draw[black, fill=black] (u) circle (5pt);
 

 \end{scope}


==> matching_distance/Push.tex <==
\begin{scope}[scale =0.5]

%axes
 \coordinate (oo) at (0,0);
 \coordinate (ox) at (9,0); 
 \coordinate (oy) at (0, 9);  
   \draw[->, ultra thick](oo) -- (ox) ;
  \draw[->, ultra thick ](oo) --(oy); 

 
\begin{scope}[xshift = -1cm, yshift = -1cm]

 % 
 \coordinate (u) at (3,3);
 \coordinate (uy) at ($(u) + (5,0)$);
 \coordinate (ux) at ($(u) + (0,5)$);
 \coordinate (nn) at (8,8); 
 
 
\coordinate (Lu) at (6.6,3);
\coordinate (L) at ($(Lu)-(45:4)$);
\coordinate (LL) at ($(Lu) + (45:3)$);

 % u
  \draw[black, fill=black] (u) circle (5pt);
  \node[anchor=north] at (u) { $u$};
 \draw[dashed ](u) -- (ux) ;
  \draw[dashed ](u) -- (uy) ;
  
  % positive cone 
\fill [fill = gray, fill opacity=0.2] (u) rectangle (nn);

  %line 
  \draw[orange]  (L)--(LL);
\node[anchor=north west ] at (LL) { \color{orange}$L$};
 % push 
 \draw[black, fill=black] (Lu) circle (5pt);
 \node[anchor =  north west ] at (Lu) {$\push_L(u)$};
 \end{scope}
 
 \end{scope}


==> matching_distance/algorithm_omega_points.tex <==
\section{Algorithms and complexity}\label{sec:alg}

%\subsection{Algorithms to compute switch points }

First, we note that all candidate switch points $\omega$ can be computed by checking quadruples $u,v,w,x$ from  $C_M\cup C_N$ using formulas given in \Cref{lem:omegapts} (see also \Cref{rem:no-need-closure}).  

There will be three algorithms: \Cref{alg:3vs1}  for the case when three points push in one direction and the fourth point pushes in the other direction;  \Cref{alg:2paired-vs-2paired} for when two paired points push in one direction while the other two paired points push in the other direction; finally, \Cref{alg:2unpaired-vs-2unpaired} takes care of the remaining case. 

 All \Cref{alg:3vs1,alg:2paired-vs-2paired,alg:2unpaired-vs-2unpaired}  share the common assumption that, among the four points $u,v,w,x$, $u$ is paired to $v$, while $w$ is paired to $x$. 
 Additionally, we require that at least 3 of the points $u,v,w,x$ are distinct. 
 
 Also, in the formulas that follow, both $\delta, \eta$ depend on which of $C_M$ or $C_N$ the points $u,v,w,x$ belong to. We note that each point can belong to either of the sets, yielding for each set of $u,v,w,x$ multiple combinations of $\delta$ and $\eta$. If $u,v$ are both in $C_M$ (respectively $C_N$), then we need to set $\delta = 2$, and if they are in different sets, then  we need to set $\delta =1$. The same reasoning applies for $w,x$ and $\eta$, yielding up to four possible combinations of $\delta, \eta \in \{1,2\}$. 
 In the algorithms, this is achieved by considering the module a point comes from as a parent of the point. 
Note that it is possible that $a\in C_M\cap C_N$. In this case, $a$ admits as parents both $M$ and $N$.
 
%\robyn{this is also a footnote in the paper.}



We now analyze the three algorithms separately. 
They correspond to the cases listed as \cref{case2,case3,case4}
in the proof of \Cref{lem:omegapts}.  We do not include an algorithm for \cref{case1}, as this situation does not produce switch points. So, we are only interested in those lines of $E(A(u,v,w,x))$ that do not contain $x$. 

However,  some configurations of points $u,v,w,x$ are not feasible: computations would lead to erroneous switch points for three reasons: 
\begin{enumerate}
\item\label{issue-1}  there is no line with positive slope that separates the four points as required;  
\item\label{issue-2} the condition  $\Delta_L=0$ cannot be satisfied by any line with positive slope that separates the four points as required; 
\item\label{issue-3} the push of the given point on the lines through the candidate switch point $\omega$ does not belong to the support of the indecomposable summands of the persistence module whose bars it is supposed to switch. So we do not truly have bars in the barcode that extend till that $\omega$. 
\end{enumerate}

In what follows, we will make sure that the obtained switch points do not present issues as in \Cref{issue-1,issue-2}. As for \Cref{issue-3}, we cannot avoid it as we are not assuming any knowledge on the support of the persistence modules $M$ and $N$ and their decompositions.

\subsection{Algorithm 3vs1}\label{sec:alg3vs1}


\Cref{alg:3vs1} is used to compute switch points for all possible combinations of four points in $C_M\sqcup C_N$, the corresponding possible combinations of $\delta$ and $\eta$, and the possible choices of $A(u,v,w,x)$ leading to configurations where the point $x$ is strictly on the left (resp. right) of a line in $E(A(u,v,w,x))$ and the points $u,v,w$ on the right (resp. left) of that line, but not strictly. 
This corresponds to the case listed as \cref{case2}
in the proof of \Cref{lem:omegapts}.  



With reference to the above-listed issues in   \Cref{issue-1,issue-2,issue-3},  we will proceed as follows.  To remedy issue 1), we introduce the function \textsc{CheckPts} (see \Cref{alg:checkpts}) as a way of discarding some impossible switch points. The correctness of the function \textsc{CheckPts} is guaranteed by the following proposition which identifies when there are no lines in the equivalence class $E(A(u,v,w,x))$: this occurs when $x$ is contained in the convex hull of $u,v,w$, or when $x$ is required to push upward (resp. rightward), but it is to the left and above (resp. to the right and below) of one of the three points.  The following proposition is used to show that the function \textsc{CheckPts} will correctly determine quadruples for which there is no line that separates the four points as required.

Before stating such proposition, let us recall that the notation $E(A(u,v,w,x))$ means \lq\lq lines for which $u,v,w,x$ push in the directions specified by $A_u$, $A_v$, $A_w$, $A_x$, respectively\rq\rq.  So, if we say  $2\in A_u\cap A_v\cap A_w$, any of these could also be $\{1,2\}$, which would mean that $E(A(u,v,w,x))$ contains also lines through any of the points $u,v,w$;  instead, because we say $A_x=\{1\},$ then this  requires that $x\notin L$ for any line in $E(A(u,v,w,x))$.  

\begin{proposition}\label{prop:erroneous-config-3vs1}
Given four not necessarily distinct  points $u,v,w,x$, let us take $A_u,A_v,A_w,A_x$ to be non-empty subsets of $\{1,2\}$. The following statements hold:

\begin{enumerate}
\item If $2\in A_u\cap A_v\cap A_w$ and $ A_x=\{1\}$, i.e. the point $x$ is required to push strictly upwards while $u,v,w$ push rightwards, albeit not necessarily strictly,  to every line $L\in E(A(u,v,w,x))$,  then the set of lines $E(A(u,v,w,x))$ is empty if and only if there is some point $a=(a_1,a_2)$  in the convex hull of $u,v,w$ such that $x_1\le  a_1$ and $x_2\ge a_2$. 
%
\item If $1\in A_u\cap A_v\cap A_w$ and $ A_x=\{2\}$, i.e. the point $x$ is required to push strictly rightwards while $u,v,w$ push upwards, albeit not necessarily strictly, to every line $L\in E(A(u,v,w,x))$,  then the set of lines $E(A(u,v,w,x))$   is empty if and only if there is some point $a=(a_1,a_2)$ in the convex hull of $u,v,w$, such that $x_1\ge  a_1$ and $x_2\le a_2$.
%
\item   If $2\in A_u\cap A_v\cap A_w$ and $ A_x=\{1,2\}$, i.e. the point $x$ is required to belong to every line $L\in E(A(u,v,w,x))$   while $u,v,w$ push rightwards onto them, and possibly $x$ coincides with any of $u,v,w$,  then the set of lines  $E(A(u,v,w,x))$   is empty if and only if there is some point $a=(a_1,a_2)$  in the convex hull of $u,v,w$ such that $x_1\le  a_1$, $x_2\ge  a_2$, and $x\ne a$.
%
\item  If $1\in A_u\cap A_v\cap A_w$ and $ A_x=\{1,2\}$, i.e. the point $x$ is required to belong to every line $L\in E(A(u,v,w,x))$   while $u,v,w$ push upwards onto them, and possibly $x$ coincides with any of $u,v,w$,  then the set of lines  $E(A(u,v,w,x))$   is empty if and only if there is some point $a=(a_1,a_2)$  in the convex hull of $u,v,w$ such that $x_1\ge  a_1$, $x_2\le  a_2$, and $x\ne a$.

\end{enumerate}
\end{proposition}


\begin{proof}
\input{matching_distance/proofs/erroneous-config-3vs1}
\end{proof}

%%%% moved inside the proof
%\end{figure}





Note that \Cref{prop:erroneous-config-3vs1} is used to determine which quadruples $u,v,w,x$ cannot be separated by a line with positive slope.  Using this proposition, \Cref{alg:checkpts} is used to avoid computing certain ``impossible" omega points that would be generated by these quadruples.  

However, it may be the case that a quadruple can be separated appropriately by a line with positive slope, but that no such line satisfies $\Delta_L=0$ (issue 2). To remedy this issue,  \Cref{prop:omega-C} determines these quadruples; we would like to exclude  we would like to exclude the omega points obtained from such quadruples from the overall set of omega points returned by \Cref{alg:3vs1}. 

%For the meaning of the notations $A_u$, $A(u,v,w,x)$, $ E(A(u,v,w,x))$ we refer the reader to \Cref{notation:A(U)}.

\begin{proposition}\label{prop:omega-C}
Given  three not necessarily distinct   points $u,v,w$, and a point $x\ne w,u,v$, let us take $A_u,A_v,A_w,A_x$ to be non-empty subsets of $\{1,2\}$ for which the set $ E(A(u,v,w,x))$ is non-empty. 

\begin{enumerate}
\item When $2\in A_u\cap A_v\cap A_w$ and $A_x=\{1\}$, i.e. the point $x$ is required to push  upwards while $u,v,w$ push rightwards to every line $L\in E(A(u,v,w,x))$, letting $\omega$ be given by \cref{eq:omega-1} or  \cref{eq:omega-3} (so that $\omega_1=x_1$), $E(A(u,v,w,x))$ contains some lines $L$ for which  $\Delta_L(u, v, w, x; \delta,\eta)=0$ if and only if
\begin{itemize} 
\item $\omega_2>x_2$ and, moreover,
\item there is no point $a=(a_1,a_2)$ in the convex hull of $u,v,w$  with $\omega_1\le a_1$, $\omega_2\ge a_2$, and $a\ne \omega$.
\end{itemize}
%In particular, if $x_1>\bar a_1$, then it is enough that $\omega_2>x_2$.
%
\item When $1\in A_u\cap A_v\cap A_w$ and $ A_x=\{2\}$, i.e.~the point $x$ is required to push  rightwards while $u,v,w$ push upwards to every line $L\in E(A(u,v,w,x))$, letting   $\omega$ be given by \cref{eq:omega-2} or \cref{eq:omega-4}, $E(A(u,v,w,x))$ (so that $\omega_2=x_2$) contains some lines $L$ for which  $\Delta_L(u, v, w, x; \delta,\eta)=0$ if and only if 
\begin{itemize}
    \item $\omega_1>x_1$ and, moreover,
\item there is no point $a=(a_1,a_2)$ in the convex hull of $u,v,w$  with $\omega_1\ge a_1$, $\omega_2\le a_2$, and $a\ne \omega$.
\end{itemize}
\end{enumerate} 
\end{proposition}

\begin{proof}
\input{matching_distance/proofs/omega-C}
\end{proof}  

We are able to use \Cref{alg:checkpts} to partially check the conditions of \Cref{prop:omega-C}, as the following result shows.


\begin{proposition}\label{prop:omega-D}
Given  three not necessarily distinct   points $u,v,w$,  the following statements are equivalent:
\begin{itemize} 
\item there is no point $a=(a_1,a_2)$ in the convex hull of $u,v,w$  with $\omega_1\le a_1$, $\omega_2\ge a_2$, and $a\ne \omega$.
\item $\mathrm{CheckPts}(u,v,w,\omega, \mathrm{Below})=\mathrm{True}$, or $\mathrm{CheckPts}(u,v,w,\omega, \mathrm{Below})=\mathrm{False}$ and $\omega\in \partial\mathrm{convhull}(u,v,w)$.
\end{itemize}
Similarly, the following statements are equivalent:
\begin{itemize} 
\item there is no point $a=(a_1,a_2)$ in the convex hull of $u,v,w$ with $\omega_1\ge a_1$, $\omega_2\le a_2$, and $a\ne \omega$.
\item $\mathrm{CheckPts}(u,v,w,\omega, \mathrm{Above})=\mathrm{True}$, or $\mathrm{CheckPts}(u,v,w,\omega, \mathrm{Above})=\mathrm{False}$ and $\omega\in \partial\mathrm{convhull}(u,v,w)$.
\end{itemize}
\end{proposition}

\begin{proof}
\input{matching_distance/proofs/omega-D}
\end{proof}

We observe that if $\omega$ is on the boundary of the convex hull of $u,v,w$, then the line  through $\omega$ separating $u,v,w$ from $x$ for which $\Delta_L=0$ passes through two of the points $u,v,w$. Thus, this line is eventually generated even if $\omega$ is not added to the set of switch points as it is a line through two critical points. So, this omega point is superfluous and does not need to be added to the set of switch points. \Cref{prop:omega-C,prop:omega-D}, and the last observation justify the call of \Cref{alg:omega-C} by \Cref{alg:3vs1} to reject erroneous or superfluous omega points. 

 




%%%%%%%%%%
Finally, in \Cref{alg:3vs1}, given a configuration of points $c_1,c_2,c_3,c_4$ extracted from $C_M\sqcup C_N$, such that 3 are distinct, we label them as $x,u,v,w$ so that $x$ and $w$ are distinct, and can then relabel (if necessary) the remaining two points to ensure that $p_L(u)>p_L(v)$.  To determine which switch point is generated, we must also determine the sign of $p_L(x)-p_L(w)$.  The following proposition can be used to determine, from $x$ and $w$, the possible signs of this difference, ensuring the correctness of lines 28--43 of  \Cref{alg:3vs1}.


\begin{proposition}\label{prop:lubparametercheck}
    Let $x,w$ be two distinct points in $C_M\cup C_N$. For every line $L$  with positive slope which separates $x$ and $w$, it holds that: 
    \begin{itemize}
    \item If $\lub(w,x)=x$, then $p_L(x)\geq p_L(w)$.
    \item If $\lub(w,x)=w$, then $p_L(x)\leq p_L(w)$.
    \item If $\lub(w,x)$ is neither $x$ nor $w$, then $p_L(x)\geq p_L(w)$ for all lines $L$ which separate $w$ and $\lub(w,x)$, and $p_{L'}(x)\leq p_{L'}(w)$ for all lines $L'$ which separate $x$ and $\lub(w,x)$.
    \end{itemize}
\end{proposition}

\begin{proof}
\input{matching_distance/proofs/lubparametercheck}
\end{proof}

The pseudo-code of \Cref{alg:3vs1} is given in \Cref{app:pseudo-code}.

%%%%%%%%%%%%%% 2paired-vs-2paired
\subsection{Algorithm 2paired-vs-2paired}\label{sec:alg-2paired-vs-2paired}

\Cref{alg:2paired-vs-2paired} is used to compute switch points for all possible combinations of four points in $C_M\sqcup C_N$,  the corresponding possible combinations of $\delta$ and $\eta$, and the possible choices of $A(u,v,w,x)$ leading to configurations where two paired points lie strictly on the left of a line in $E(A(u,v,w,x))$ and the other two paired points lie strictly on the right of that line.  This corresponds to the case listed as \cref{case3} in the proof of \Cref{lem:omegapts}. 

If a quadruple of distinct points generates a switch point $\omega$ with this configuration,  that point is the point at infinity given by \Cref{eq:omega-ter}: with the appropriate labeling of the four points given in \cref{case3}, $\omega=[0,\delta(w_1-x_1),\eta(u_2-v_2)]$,  which identifies a specific slope.  Appropriate labeling refers to the fact that, given four distinct points that are separated by a line $L$ with positive slope so that two lie strictly on one side of the line and the other two lie strictly on the other side, there is exactly one way to label these points as $x,w,u,v$ so that:
\begin{itemize}
    \item $x,w$ push up to $L$ and $p_L(w)>p_L(x)$, and
    \item $u,v$ push right to $L$ and $p_L(u)>p_L(v)$.
\end{itemize}

Note that, with this labeling, the $\omega$ slope that is generated by \Cref{eq:omega-ter} is by  construction positive. 

In \cref{case3},  we saw that if $ A_u= A_v=\{2\}$ and $A_x=A_w=\{1\}$, then no switch point is generated if $x_1=w_1$ or $u_2=v_2$. Moreover, it is the case that the paired points must be distinct; otherwise, the cost of matching that pair would be zero.  Since the pairs must lie strictly on one side of the line, it is not possible that one point may simultaneously be in two pairs. So, it must be the case that all 4 points are distinct.



As in \Cref{sec:alg3vs1}, it may be the case that there is no line with positive slope that separates the four distinct points as required.  We introduce the function \textsc{CheckPts2} (see \Cref{alg:checkpts-2v2paired}) to discard these sets of points.  The correctness of this function is guaranteed by \Cref{prop:erroneous-config-2vs2pair}. 


\begin{proposition}\label{prop:erroneous-config-2vs2pair}
     Let $u,v,w,x$ be four points, with $ A_u= A_v=\{2\}$, $A_x=A_w=\{1\}$.
     Define 
     $$Q=\{(p_1,p_2)\in\RR^2|p_1
     \leq a_1 \textrm{ and } p_2\geq a_2\textrm{ for some } a\in \overline{uv}\}$$
     and 
    $$R=\{(p_1,p_2)\in\RR^2|p_1
     \geq b_1 \textrm{ and } p_2\leq b_2\textrm{ for some } b\in \overline{xw}\}.$$
     The following statements are equivalent:

     \begin{enumerate}
         \item[(i)] $R\cap Q\neq\emptyset$,
         \item[(ii)] the set of lines $E(A(u,v,w,x))$ is empty,
         \item[(iii)] there are a point $a=(a_1,a_2)$  on the line segment $\overline{uv}$ and a point $b=(b_1,b_2)$ on the line segment $\overline{xw}$ such that $(b_1\le  a_1)\wedge (b_2\ge a_2)$,
         \item[(iv)] Either $x$ or $w\in Q$, or $u$ or $v\in R.$
     \end{enumerate}
\end{proposition}


\begin{proof}
\input{matching_distance/proofs/erroneous-config-2vs2pair}
\end{proof}

More precisely, the function \textsc{CheckPts2} uses condition 4 from \Cref{prop:erroneous-config-2vs2pair} to check for erroneous quadruples of points.


We now need an analogue of \Cref{prop:omega-C,prop:omega-D}. Each set of four points generates one switch slope $\omega$ and all lines with that slope are guaranteed to have $\Delta_L(u, v, w, x; \delta,\eta)=0$.  
The following proposition determines if it is possible to split the four points appropriately with a line with that particular omega slope.  This will happen exactly when $\max\{x_2-mx_1,w_2-mw_1\}<\min\{u_2-m u_1,v_2-mv_1\}$, i.e, when the $y$-intercepts of the lines through $u,v,w,x$ are ordered appropriately.



% \robyn{if both slopes are positive, then we have a slope range given by endpoints which are the slopes of the two segments uv and wx.  when uv is pos, xw is negative, then the bounds are max{0,slope ux} and min{slope uv, slope xv,}}

\begin{proposition}\label{prop:omega-2pv2p}
 Given four distinct points $u,v,w,x$, let us take $A_u=A_v=\{2\}$ and $A_w=A_x=\{1\}$ (i.e.~the points $w,x$ are required to push  upwards while $u,v$ push rightwards to every line $L\in E(A(u,v,w,x))$). 
 Let us assume that the set $ E(A(u,v,w,x))$ is non-empty. Without loss of generality, let us also assume that $p_L(u)>p_L(v)$ and $p_L(w)>p_L(x)$. 
 Then, for every $\eta,\delta\in\{1,2\}$, letting $m=\frac{\delta(w_1-x_1)}{\eta(u_2-v_2)}$ be the slope identified by $\omega$ as given in \cref{eq:omega-ter},   the equivalence class $E(A(u,v,w,x))$ contains some lines $L$ \robyn{with positive slope} for which  $\Delta_L(u, v, w, x; \delta,\eta)=0$ if and only if 
 \begin{equation}\label{eq:omega-2pv2p}
     \max\{x_2-mx_1,w_2-mw_1\}<\min\{u_2-m u_1,v_2-mv_1\}
 \end{equation}
\end{proposition}

\begin{proof}
\input{matching_distance/proofs/omega-2pv2p}
\end{proof}

The pseudo-code of \Cref{alg:2paired-vs-2paired} can be found in \Cref{app:pseudo-code}.

%%%%%%%%%%%%%%%
\subsection{Algorithm 2unpaired-vs-2unpaired}\label{sec:alg-2unpaired-vs-2unpaired}

\Cref{alg:2unpaired-vs-2unpaired} is used to compute switch points for all possible combinations of four points in $C_M\sqcup C_N$, with at least three of them distinct,  the corresponding possible combinations of $\delta$ and $\eta$, and the possible choices of $A(u,v,w,x)$ leading to configurations where a line in $E(A(u,v,w,x))$ splits both pairs; i.e., one point of a pair is strictly on the left, and one point is strictly on the right. This corresponds to the case listed as \cref{case4}
in the proof of \Cref{lem:omegapts}. We may assume without loss of generality  that $u$ and $w$ lie to the left of the line, and that $v$ and $x$ lie to its right.

Like in \Cref{sec:alg-2paired-vs-2paired},  some configurations of points are not feasible. To determine which configurations have no line with positive slope that separates the four points as required, we can use again the function \textsc{CheckPts2} (\Cref{alg:checkpts-2v2paired}) simply by changing the roles of $u,v,w,x$, that is calling $\mathrm{CheckPts2}(x,v,w,u)$ instead of $\mathrm{CheckPts2}(x,w,u,v)$.

If the configuration is feasible, always assuming that the matched pairs are $u,v$ and $x,w$, and also assuming without loss of generality that $u$ and $w$ lie to the left of the line and that  $v$ and $x$ lie to its right,  we can compute the candidate switch points with the following formulas:
\begin{itemize}
%    
\item If  $p_L(u)\geq p_L(v)$ and $p_L(w)\geq p_L(x)$, or $p_L(u)\leq p_L(v)$ and $p_L(w)\leq p_L(x)$, and moreover
%
\begin{itemize}
    \item $\delta=\eta$, and $x_1= v_1$ or $u_2= w_2$, then no switch point is generated;
    \item $\delta=\eta$,  $x_1\neq v_1$, and $u_2\neq w_2$, then the omega slope $\omega= [0:v_1-x_1:u_2-w_2]$ is generated, by \Cref{eq:omega-quater}; 
    \item  $\delta\ne \eta$, then the proper point $\omega=\left(\frac{\eta v_1-\delta x_1}{\eta-\delta},\frac{\eta u_2-\delta w_2}{\eta-\delta}\right)$ is generated, by \Cref{eq:omega-5}.
\end{itemize}
%
\item If  $p_L(u)\geq p_L(v)$ and $p_L(w)\leq p_L(x)$, or  $p_L(u)\leq p_L(v)$ and $p_L(w)\geq p_L(x)$, then the proper omega point 
$\omega =\left(\frac{\eta v_1+\delta x_1}{\eta+\delta},\frac{\eta u_2+\delta w_2}{\eta+\delta}\right)$ is generated,
by \Cref{eq:omega-6}.
\end{itemize}


Because in the case under examination where among the four points matched pairs do not lie completely on one side of the line $L$,   we may fix the labels $u,v,w,x$ to identify with $u$ and $w$ those on the left of $L$ and by $v$ and $x$ those on the right. However, depending on $L$,  both $p_L(u)\geq p_L(v)$ and $p_L(u)\leq p_L(v)$  can occur (similarly for $x,w$). To decide which one occurs, we apply \Cref{prop:lubparametercheck} in lines 28 and 42  of \Cref{alg:2unpaired-vs-2unpaired}. 

It may also be the case that the condition $\Delta_L=0$ cannot be satisfied by any line with positive slope through $\omega$. In the case when $\omega$ is a point at infinity, this issue can be addressed as in  \Cref{prop:omega-2pv2p} with the roles of $w$ and $v$ switched.  The only assumption from \Cref{prop:omega-2pv2p} that is not satisfied is that we are not guaranteed that $p_L(u)>p_L(v)$ and $p_L(w)>p_L(x)$, which, in the proof, ensures that any line with slope given by $\omega$ has positive slope.  So, in \Cref{alg:2unpaired-vs-2unpaired} we discard any $\omega$ points which generate lines with non-positive slope, and then check a modified version of \Cref{eq:omega-2pv2p}.


When $\omega$ is a proper point, we may determine when $\Delta_L=0$ for a line with positive slope through $\omega$ by considering the following two lines: the line through $\omega$ and $u$, and $\omega$ and $w$.  If either of these lines separates the points correctly, then we can rotate this line slightly to obtain a line for which $\Delta_L=0$.  If neither of these lines separates the points correctly, then there is no line through $\omega$ which has $\Delta_L=0$. This idea is formalized by the following proposition.

\begin{proposition}\label{prop:omega-2uv2u}
 Given four points $u,v,w,x$, let us take $A_u=A_w=\{2\}$ and $A_v=A_x=\{1\}$ (i.e.~the points $v,x$ push  upwards while $u,w$ push rightwards to every line $L\in E(A(u,v,w,x))$). Let us assume that the set $ E(A(u,v,w,x))$ is non-empty. Let $\omega$ be the point generated by $x,v,u,w$ by \cref{eq:omega-5} or \cref{eq:omega-6}. Partition $\RR^2$ into quadrants with respect to $\omega$ in the following way:
\[
\begin{split}
    Q_1&=\{(p_1,p_2)\in\RR^2|p_1>\omega_1 \textrm{ and }p_2>\omega_2 \}\\
    Q_2&=\{(p_1,p_2)\in\RR^2|p_1\leq\omega_1 \textrm{ and }p_2\geq\omega_2 \}\\
    Q_3&=\{(p_1,p_2)\in\RR^2|p_1<\omega_1 \textrm{ and }p_2<\omega_2 \}\\
    Q_4&=\{(p_1,p_2)\in\RR^2|p_1\geq\omega_1 \textrm{ and }p_2\leq\omega_2 \}\\    
\end{split}
\]

Then:
\begin{enumerate}
    \item If $\omega\in\{x,v,u,w\}$, then there is no line through $\omega$ in $E(A(u,v,w,x))$.
    \item If either $x$ or $v$ is in $Q_2$, or $u$ or $w$ is in $Q_4$, then there is no line through $\omega$ in $E(A(u,v,w,x))$.
    \item If  $x$, $v$ are in $Q_4$ and $u$, $w$ are in $Q_2$, and $\omega\notin\{x,v,u,w\}$, then all lines through $\omega$ with positive slope are in $E(A(u,v,w,x))$.
    \item If $x,v\notin Q_2$, $u,w\notin Q_4$, and at least one of $x,v,u,w$ is in $Q_1$ or $Q_3$, denote $P=\{v,x\}\cap (Q_1 \cup Q_3)$ and $S=\{u,w\}\cap (Q_1 \cup Q_3)$. 
    Then for every $c\in \{u,v,x,w\}\cap(Q_1\cup Q_3) = P\cup S$, let $0\le m_c\le \infty$ be the slope of the line through $\omega$ and $c$, and 
    \[
    \mathrm{sign}_1(c)=\left\{\begin{array}{ll} +1 & \mbox{if $c\in Q_1$}\\-1 & \mbox{if $c\in Q_3$}\end{array}\right.
    \]

    \[
    \mathrm{sign}_2(c)=\left\{\begin{array}{ll} +1 & \mbox{if $c\in P$}\\-1 & \mbox{if $c\in S$.}\end{array}\right.
    \]
    
    Then there is a line with positive slope through $\omega$ in $E(A(u,v,w,x))$ if and only if there exists $0<m<\infty$ such that $$\mathrm{sign}_1(c)\mathrm{sign}_2(c)m_c < \mathrm{sign}_1(c)\mathrm{sign}_2(c)m$$ for every $c\in \{u,v,x,w\}\cap(Q_1\cup Q_3)$.
    
    % consider the set of lines through $\omega$ and the points of $u,v,x,w$ which are in either $Q_1$ or $Q_3$ (there is at least one and at most four such lines.)  If at least one of these lines has the property that $x,v$ push up to and $u,w$ push right to (or possibly lie on) the line, then there is a line with positive slope through $\omega$ in $E(A(u,v,w,x))$.  Otherwise, there is no line through $\omega$ with positive slope in $E(A(u,v,w,x))$. 
    % \barbara{I think we need to refine this third case regarding points from $\{u,v,x,w\}$ lying on a line though $\omega$ and another point from $\{u,v,x,w\}$. For example, in the case where $v$ lies on $L_x$ and $u$ and $w$ push to the right onto $L_x$, it is important to know which quadrant $v$ lies in: If $m_u > m_x = m_v > m_w$ and $x,u \in Q_1, w\in Q_3$, then a desired line exists if $v \in Q_1$, but not if $v \in Q_3$. Each point of $\{u,v,x,w\}$ that lies in $Q_1\cup Q_3$ is associated with an open subset of the positive reals (the slopes of lines through $\omega$ that have the point on the desired side). Two such subsets can share a boundary (as the subsets corresponding to $x$ and $v$ in the example above), but not overlap (as in the case where $x \in Q_1$ and $v \in Q_3$ in the example above). } 
    % \claudia{I agree with Barbara, but how can we ensure this in a concise way? Maybe like this: for every $c\in \{u,v,x,w\}\cap(Q_1\cup Q_3)$, let $0\le m_c\le \infty$ be the slope of the line through $\omega$ and $c$, and 
    % $$\mathrm{sign}(c)=\left\{\begin{array}{ll} +1 & \mbox{if $c\in Q_1$}\\-1 & \mbox{if $c\in Q_3$}\end{array}\right.$$
    % Then there is a line with positive slope through $\omega$ in $E(A(u,v,w,x))$ if and only if there exists $0<m<\infty$ such that $  \mathrm{sign}(c)m_c\le \mathrm{sign}(c)m$  for every $c\in \{u,v,x,w\}\cap(Q_1\cup Q_3)$.
    % }
\end{enumerate}

\end{proposition}



\begin{proof}
\input{matching_distance/proofs/omega-2uv2u}
\end{proof}	  

% Based on \Cref{prop:omega-2uv2u}, in \Cref{alg:checkomega3} we may determine if a proper $\omega$ point satisfies the condition $x,v$ pushes up and $u,w$ push right to at least one of the lines $L_u$ and $L_w$ by ensuring that at least one of the following systems of inequalities is verified:   

\subsection{The matching distance algorithm}

Having developed  algorithms for the explicit computations of the switch points in the previous sections, the algorithm to compute the matching distance between the persistence modules $M$ and $N$  based on the framework in this paper can be now described by the following main steps, assuming $C_M$ and $C_N$ are given: 
\begin{enumerate}
    \item Identify the critical values in $\closure C_M$ and $\closure C_N$;
    \item Compute the set of switch-points $\Omega$ using the results from \Cref{sec:alg3vs1,sec:alg-2paired-vs-2paired,sec:alg-2unpaired-vs-2unpaired};
    \item Compute all the lines through pairs of points in $\closure C_M\cup \closure C_N\cup{\Omega}$ and lines of diagonal slope through at least one point of $\closure C_M\cup \closure C_N\cup{\Omega}$ and for each line do:
    \begin{enumerate}
    \item Compute the persistence diagrams of the restrictions of $M$ and $N$ to that line;
    \item Compute their bottleneck distance together with its corresponding weight;
    \end{enumerate}
    \item Output the maximum of the weighted bottleneck distances.   
\end{enumerate}

\subsection{Complexity analysis}
\robyn{perhaps complexity analysis can be: starting with a number of critical values, how many omega points will we get?  discuss the size of omega}

\claudia{I'm drafting the time complexity analysis. It should be carefully reviewed by those more expert than me. Also, it would be nice to say something about the space complexity.}

Let $m=|C_M|$, $n=|C_N|$, $h=|\Omega|$. For simplicity, we also set $r=m+n$ and $p=m+n+h$. In the worst case,  the order of $|\Omega|$ is   $h\approx 250 {r \choose{4}}$. Indeed,  for each choice of four points extracted  from $C_M\cup C_N$,  we have 
\begin{itemize}
    \item in the 1-vs-3 case, we have $4$ choices for $x$, 3 choices  for $w$, 2 choices for the position above or below the line, 4 choices for the combinations of $\delta$ and $\eta$, each potentially giving a switch point, totaling a worst-case scenario of 96 switch points.
    \item in the 2paired-vs-2paired case, we have  $4$ choices for $x$, 3 choices for $w$, 4 choices for the combinations of $\delta$ and $\eta$, each potentially giving a switch point, totaling for a worst-case scenario of 48 switch points.
    \item in the 2unpaired-vs-2unpaired case, we have  $4$ choices for $x$, 3 choices for $w$, 4 choices for the combinations of $\delta$ and $\eta$, each potentially giving 2 switch points, totaling for a worst-case scenario of 96 choices.
\end{itemize}   
Thus, in the worst case, the order of $p$ is $O(r^4)$.

The  time complexity  of computing the least upper bound of two points of $\RR^2$ is $O(1)$, so doing it for all pairs of points of a set with $n$ points is $O(n^2)$. From this we can deduce the complexity of step 1 in terms of $m$ and $n$ is $O(m^2+n^2)$.\\

\claudia{I'm skipping the complexity analysis of algorithms in \Cref{sec:alg3vs1,sec:alg-2paired-vs-2paired,sec:alg-2unpaired-vs-2unpaired} for now.}\\

The time complexity of computing all the possible lines through two points in a set of $p$ points is $O(p^2)=O(r^8)$.\\

The time complexity of computing the persistence diagram of the restriction of $M$ and $N$) to a line is $O(m^\mu+n^\mu)$, where $\mu\approx 2.37$ is the matrix multiplication constant. That of computing the bottleneck distance in a set with $s$ points of the plane is $O(s^{\mu/2}\log s)$ \cite{Katz2023}. For us, $s$ can be assumed to be in the order of $m+n$, yielding $O((m+n)^{\mu/2}\log(m+n))$ for the cost of computing the bottleneck distance for a line. Thus, the sum of the costs of steps (a) and (b) can be evaluated to be no more than $O(r^\mu)$.

Because this has to be repeated for each line, whose number is $O(r^8)$, we get the total time complexity for step 4 bounded by $O(r^{8+\mu})$, which dominates that of the previous steps. 

In conclusion, the time complexity of our method is roughly $O(r^{11})$, which is in line with that of \cite{lesnick2020computing} and higher than that of \cite{Bjerkevik2021} which is $O(r^5\log^3r)$.


\subsection{Experimental results}



==> matching_distance/figures/2v2pairedUVnegslope.tex <==
\begin{scope}[scale =0.5]


 %points u,v
 \coordinate (u) at (1,2);
 \coordinate (v) at (6,0);
\coordinate (r2) at (6, 6);
\coordinate (r3) at (-2,0);
\coordinate (r1) at (-2,6);

\fill[fill=red!10]    (r3)-- (v)--(r2)--(r1);

%draw points
\draw[red, fill=red] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[red, fill=red] (v) circle (5pt);
  \node[anchor=south] at (v) { $v$};

\draw[red, dashed]  (v)--(r2);
\draw[red, dashed]  (r3)--(v);
\draw[red]  (u)--(v);

\node[anchor=north west ] at (3,4) { \color{red}$Q$};

 \end{scope}


==> matching_distance/figures/2v2pairedUVposslope.tex <==
\begin{scope}[scale =0.5]


 %points u,v
 \coordinate (v) at (1,0);
 \coordinate (u) at (6,2);
\coordinate (r2) at (6, 6);
\coordinate (r3) at (-2,0);
\coordinate (r1) at (-2,6);

\fill[fill=red!10]    (r3)-- (v) -- (u)--(r2)--(r1);

%draw points
\draw[red, fill=red] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[red, fill=red] (v) circle (5pt);
  \node[anchor=south] at (v) { $v$};

\draw[red, dashed]  (u)--(r2);
\draw[red, dashed]  (r3)--(v);
\draw[red]  (u)--(v);

\node[anchor=north west ] at (3,4) { \color{red}$Q$};

 \end{scope}


==> matching_distance/figures/2v2pairedXWnegslope.tex <==
\begin{scope}[scale =0.5]


 %points u,v
 \coordinate (w) at (6,0);
 \coordinate (x) at (1,2);
\coordinate (r2) at (10, 2);
\coordinate (r3) at (1,-4);
\coordinate (r1) at (10,-4);

\fill[fill=blue!10]    (r3)-- (x)--(r2)--(r1);

%draw points
\draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};
   \draw[blue, fill=blue] (x) circle (5pt);
  \node[anchor=south] at (x) { $x$};

\draw[blue, dashed]  (x)--(r2);
\draw[blue, dashed]  (r3)--(x);
\draw[blue]  (w)--(x);

\node[anchor=north west ] at (4,-0) { \color{blue}$R$};

 \end{scope}


==> matching_distance/figures/2v2pairedXWposslope.tex <==
\begin{scope}[scale =0.5]


 %points u,v
 \coordinate (x) at (1,0);
 \coordinate (w) at (6,2);
\coordinate (r2) at (10, 2);
\coordinate (r3) at (1,-4);
\coordinate (r1) at (10,-4);

\fill[fill=blue!10]    (r3)-- (x) -- (w)--(r2)--(r1);

%draw points
\draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};
   \draw[blue, fill=blue] (x) circle (5pt);
  \node[anchor=south] at (x) { $x$};

\draw[blue, dashed]  (w)--(r2);
\draw[blue, dashed]  (r3)--(x);
\draw[blue]  (w)--(x);

\node[anchor=north west ] at (4,-0) { \color{blue}$R$};

 \end{scope}


==> matching_distance/figures/Omega2.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (5,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
%\coordinate (c5) at ($(c2)+ (0,2)$);
  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
 \coordinate (L) at ($(3.5,0)-(40:1)$);
  \coordinate (LL) at ($(L)+(40:13)$); 
  

  \coordinate (L') at ($(3.5,0)-(55:1)$);
  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
 % \node[anchor=north] at (c1) { $c_1$};
   \draw[red, fill=red] (c2) circle (5pt);
  %\node[anchor=north] at (c2) { $c_2$};
  %\draw[black, fill=black] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
%  \node[anchor=north] at (c4) { $c_4$};
  
%\draw[dashed ](c1) -- (C);
%\draw[dashed ](c1) -- (D);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
\draw[orange, thick]  (L)--(LL);
\node[anchor=north west ] at (LL) { \color{orange}$L$};


\draw[orange, thick]  (L')--(LL');
\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> matching_distance/figures/Omega3.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (5,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
\coordinate (c5) at ($(c2)+ (0,2)$);
  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
 \coordinate (L) at ($(3.5,0)-(40:1)$);
  \coordinate (LL) at ($(L)+(40:13)$); 
  

  \coordinate (L') at ($(3.5,0)-(55:1)$);
  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
 % \node[anchor=north] at (c1) { $c_1$};
   \draw[red, fill=red] (c2) circle (5pt);
  %\node[anchor=north] at (c2) { $c_2$};
  %\draw[blue, fill=blue] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
%  \node[anchor=north] at (c4) { $c_4$};
\draw[green, fill=green] (c5) circle (5pt);
\node[anchor=north] at (c5) { $\omega$}; 
  
%\draw[dashed ](c1) -- (C);
%\draw[dashed ](c1) -- (D);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
\draw[orange, thick]  (L)--(LL);
\node[anchor=north west ] at (LL) { \color{orange}$L$};


\draw[orange, thick]  (L')--(LL');
\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> matching_distance/figures/Omega4.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 \coordinate (c1) at (3,3);
 \coordinate (c2) at ($(c1) + (7,0)$);
 \coordinate (c3) at ($(c1) + (0,4)$);
 \coordinate (c4) at ($(c3)+ (5,0)$); 
\coordinate (c5) at ($(c2)+ (0,2)$);
\coordinate (e) at ($(c1)+ (2.5,2)$);
\coordinate (f) at ($(e)+(8,0)$); 
\coordinate (g) at ($(c2)+(0,6)$);  
 
% \coordinate (C) at ($(c1)+ (7,0)$); 
% \coordinate (D) at ($(c1) + (0,7)$); 
% \coordinate (E) at ($(c3) + (7,0)$); 
% \coordinate (F) at ($(c2) + (0,7)$);
 
% \coordinate (L) at ($(3.5,0)-(40:1)$);
%  \coordinate (LL) at ($(L)+(40:13)$); 
%  
%
%  \coordinate (L') at ($(3.5,0)-(55:1)$);
%  \coordinate (LL') at ($(L')+(55:13)$); 

 % axes 
%  \draw[->, ultra thick](oo) -- (ox) ;
%  \draw[->, ultra thick ](oo) --(oy); 


 % Critical Set 
  \draw[blue, fill=blue] (c1) circle (5pt);
  \node[anchor=north] at (c1) { $a$};
   \draw[red, fill=red] (c2) circle (5pt);
  \node[anchor=north] at (c2) { $b$};
  %\draw[blue, fill=blue] (c3) circle (5pt);
 % \node[anchor=north] at (c3) { $c_3$};
 \draw[blue, fill=blue] (c4) circle (5pt);
  \node[anchor=north] at (c4) { $c$};
\draw[green, fill=green] (c5) circle (5pt);
\node[anchor=north] at (c5) { $\omega$}; 
\draw[black, fill=black] (e) circle (5pt);
\node[anchor=north] at (e) { $e$}; 
 
\draw[dashed ](c1) -- (c4);
\draw[dashed ](e) -- (f);
\draw[dashed ](c2) -- (g);
%\draw[dashed ](c3) -- (E);
%\draw[dashed ](c2) -- (F);

  

%lines 
%\draw[orange, thick]  (L)--(LL);
%\node[anchor=north west ] at (LL) { \color{orange}$L$};


%\draw[orange, thick]  (L')--(LL');
%\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (c1_L) at ($(c1) + (0,1.5)$);
%\coordinate (c2_L) at ($(c3) + (2.5,0)$);
%\coordinate (c3_L) at ($(c4) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (c1_L) circle (5pt);
%  \node[anchor=north west] at (c1_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (c2_L) circle (5pt);
%  \node[anchor=south ] at (c2_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (c3_L) circle (5pt);
%\node[anchor=south east] at (c3_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (c1_L2) at ($(c1) + (0,1.6)$);
%\coordinate (c2_L2) at ($(c3) + (3.5,0)$);
%\coordinate (c3_L2) at ($(c4) + (0,1)$);
% 
% \draw[red, fill=red] (c1_L2) circle (5pt);
%  \node[anchor=south east ] at (c1_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (c2_L2) circle (5pt);
%  \node[anchor=north] at (c2_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (c3_L2) circle (5pt);
%\node[anchor=north west] at (c3_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> matching_distance/figures/OmegaFrom3Points.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (10,0); 
 \coordinate (oy) at (0, 10); 
 
 \coordinate (u) at (1,2);
 \coordinate (w) at ($(u)+ (4,4)$); 
 \coordinate (miduw) at ($(u)+ (2,2)$);
 
 \coordinate (v) at (6,0);
 %\coordinate (x) at ($(u) + (0,4)$);
  
\coordinate (omega) at ($(v)+ (0,4)$);

\coordinate (f) at ($(miduw)+(8,0)$); 
\coordinate (g) at ($(v)+(0,8)$);  
 
    \coordinate (ue) at ($(u)+ (10,0)$); 
    \coordinate (we) at ($(w)+ (6,0)$);   
       \coordinate (ve) at ($(v)+ (0,8)$); 
   % \coordinate (xe) at ($(x)+ (0,6)$);   
  \coordinate (L) at ((12,8);
  
   % \coordinate(pv) at (2,1.3333);
    \coordinate(pu) at (3,2);
      \coordinate(pw) at (9,6);
     %   \coordinate(px) at (10,6.66666);


%\draw[red, fill=red] (pv) circle (5pt);
%\draw[red, fill=red] (px) circle (5pt);

 
\draw[dashed ](u) -- (w);
\draw[dashed ](miduw) -- (f);
\draw[dashed ](v) -- (g);
%\draw[dashed ](miduw) -- (g);

\draw[gray,dashed ](u) -- (ue);
\draw[gray, dashed ](w) -- (we);
\draw[gray,dashed ](v) -- (ve);
%\draw[gray, dashed ](x) -- (xe);


%\draw[dashed ](x) -- (miduw);
%\draw[dashed ](v) -- (F);

  

%lines 

\draw[orange, thick]  (oo)--(L);
\node[anchor=north west ] at (L) { \color{orange}$L$};

\draw [line width=0.5mm, red ]   (omega)--(pu);
\draw [line width=0.5mm, red ]   (pw)--(omega);

 % Critical Set 
  \draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v=x$};
  %\draw[blue, fill=blue] (x) circle (5pt);
 % \node[anchor=north] at (x) { $c_3$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};
  
 

\draw[black, fill=black] (miduw) circle (5pt);
\node[anchor=south] at (miduw) { $m$}; 

%\draw[orange, thick]  (L)--(LL);
%\node[anchor=north west ] at (LL) { \color{orange}$L$};
\draw[red, fill=red] (pu) circle (5pt);
\draw[red, fill=red] (pw) circle (5pt);

\draw[cyan, fill=cyan] (omega) circle (5pt);
\node[anchor=north] at (omega) { $\omega$};

%\draw[orange, thick]  (L')--(LL');
%\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (u_L) at ($(u) + (0,1.5)$);
%\coordinate (v_L) at ($(x) + (2.5,0)$);
%\coordinate (x_L) at ($(w) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (u_L) circle (5pt);
%  \node[anchor=north west] at (u_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (v_L) circle (5pt);
%  \node[anchor=south ] at (v_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (x_L) circle (5pt);
%\node[anchor=south east] at (x_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (u_L2) at ($(u) + (0,1.6)$);
%\coordinate (v_L2) at ($(x) + (3.5,0)$);
%\coordinate (x_L2) at ($(w) + (0,1)$);
% 
% \draw[red, fill=red] (u_L2) circle (5pt);
%  \node[anchor=south east ] at (u_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (v_L2) circle (5pt);
%  \node[anchor=north] at (v_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (x_L2) circle (5pt);
%\node[anchor=north west] at (x_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> matching_distance/figures/OmegaFrom4Points.tex <==
\begin{scope}[scale =0.5]


 \coordinate (oo) at (0,0);
 \coordinate (ox) at (12,0); 
 \coordinate (oy) at (0, 12); 
 
 \coordinate (u) at (3,3);
  \coordinate (w) at ($(u)+ (2,2)$); 
\coordinate (miduw) at ($(u)+(1,1)$);
 
  \coordinate (v) at (2,0); 
 \coordinate (x) at ($(v) + (8,2)$);
\coordinate (midvx) at ($(v)+(4,1)$);

\coordinate (omega) at (6,4);

\coordinate (f) at ($(midvx)+(0,7)$); 
\coordinate (g) at ($(miduw)+(8,0)$);  

   \coordinate (ue) at ($(u)+ (9,0)$); 
    \coordinate (we) at ($(w)+ (7,0)$);   
       \coordinate (ve) at ($(v)+ (0,8)$); 
    \coordinate (xe) at ($(x)+ (0,6)$);   
  \coordinate (L) at ((12,8);
  
  \coordinate(pv) at (2,1.3333);
    \coordinate(pu) at (4.5,3);
      \coordinate(pw) at (7.5,5);
        \coordinate(px) at (10,6.66666);



 
\draw[dashed ](u) -- (w);
\draw[dashed ](v) -- (x);
\draw[dashed ](midvx) -- (f);
\draw[dashed ](miduw) -- (g);
\draw[gray,dashed ](u) -- (ue);
\draw[gray, dashed ](w) -- (we);
\draw[gray,dashed ](v) -- (ve);
\draw[gray, dashed ](x) -- (xe);

%\draw[dashed ](v) -- (E);
%\draw[dashed ](x) -- (F);

  

%lines 
\draw[orange, thick]  (oo)--(L);
\node[anchor=north west ] at (L) { \color{orange}$L$};

\draw [line width=0.5mm, red ]   (pv)--(pu);
\draw [line width=0.5mm, red ]  (pw)--(px);


 % Critical Set 
  \draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (x) circle (5pt);
  \node[anchor=north] at (x) { $x$};
  \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};
  


\draw[black, fill=black] (miduw) circle (5pt);
\node[anchor=south] at (miduw) { $m_1$}; 
\draw[black, fill=black] (midvx) circle (5pt);
\node[anchor=north] at (midvx) { $m_2$}; 
\draw[red, fill=red] (pv) circle (5pt);
\draw[red, fill=red] (pu) circle (5pt);
\draw[red, fill=red] (pw) circle (5pt);
\draw[red, fill=red] (px) circle (5pt);

\draw[cyan, fill=cyan] (omega) circle (5pt);
\node[anchor=north] at (omega) { $\omega$}; 

%\draw[orange, thick]  (L')--(LL');
%\node[anchor=north west ] at (LL') { \color{orange}$L'$};


 % push L 
%\coordinate (u_L) at ($(u) + (0,1.5)$);
%\coordinate (x_L) at ($(v) + (2.5,0)$);
%\coordinate (v_L) at ($(w) + (0,2.5)$);
% 
% \draw[orange, fill=orange] (u_L) circle (5pt);
%  \node[anchor=north west] at (u_L) {\color{orange} $c_1$};
%  \draw[orange, fill=orange] (x_L) circle (5pt);
%  \node[anchor=south ] at (x_L) { \color{orange}$c_2$};
%   \draw[orange, fill=orange] (v_L) circle (5pt);
%\node[anchor=south east] at (v_L) {\color{orange} $c_3$};
% 
 %push L'
%\coordinate (u_L2) at ($(u) + (0,1.6)$);
%\coordinate (x_L2) at ($(v) + (3.5,0)$);
%\coordinate (v_L2) at ($(w) + (0,1)$);
% 
% \draw[red, fill=red] (u_L2) circle (5pt);
%  \node[anchor=south east ] at (u_L2) { \color{red}$d_1$};
%  \draw[red, fill=red] (x_L2) circle (5pt);
%  \node[anchor=north] at (x_L2) { \color{red}$d_2$};
%   \draw[red, fill=red] (v_L2) circle (5pt);
%\node[anchor=north west] at (v_L2) { \color{red}$d_3$};
%
%%% labels
%\coordinate (Critical) at ($(-5,4) -(0,0)$); 
% \draw[black, fill=black] (Critical) circle (5pt);
%\node[anchor = west] at (Critical) {$\text{  }\closure{C}$};
%
%\coordinate (push1) at ($(-5,3) -(0,0)$); 
% \draw[orange, fill=orange] (push1) circle (5pt);
%\node[anchor = west] at (push1) {$\text{  }\mathrm{Push}_L(\closure{C})$};
%
% \coordinate (push2) at ($(-5,2) -(0,0)$); 
% \draw[red, fill=red] (push2) circle (5pt);
%\node[anchor = west] at (push2) {$\text{  }\mathrm{Push}_{L'}(\closure{C})$};
 
 \end{scope}


==> matching_distance/figures/xPushUpConvexHullExample1.tex <==
\begin{scope}[scale =0.5]


% \coordinate (oo) at (0,0);
 %\coordinate (ox) at (10,0); 
 %\coordinate (oy) at (0, 10); 

 %points u,v,w,x
 \coordinate (u) at (1,2);
 \coordinate (w) at ($(u)+ (4,4)$); 
 \coordinate (v) at (6,0);
 \coordinate (x) at (9,0.5);
  \coordinate (x') at (4,-2);
  

%draw points
\draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v=\bar a$};
 % \draw[blue, fill=blue] (x) circle (5pt);
 %\node[anchor=north] at (x) { $x$};
  % \draw[blue, fill=blue] (x') circle (5pt);
 %\node[anchor=north] at (x') { $x'$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};

 %convex hull 
 \draw[fill=red!10] (u) -- (v) -- (w) -- cycle;

%rotation point

%\coordinate (r) at (7.5, 0.25);
 % \draw[red, fill=red] (r) circle (5pt);

%lines
%verical
%\coordinate (l1) at (7.5,-3);
%\coordinate (l2) at (7.5, 10);
%\draw[orange, thick]  (l1)--(l2);
%\node[anchor=north west ] at (l2) { \color{orange}$L$};

%horizontal
%\coordinate (l3) at (0,-1);
%\coordinate (l4) at (10, -1);
%\draw[orange, thick]  (l3)--(l4);
%\node[anchor=north west ] at (l4) { \color{orange}$L'$};

%regions

\coordinate (r1) at (6,-3);
\coordinate (r2) at (6, 10);
\draw[red, dashed]  (r1)--(r2);
%\node[anchor=north west ] at (r2) { %\color{red}$y_1=\bar a_1$};

\coordinate (r3) at (0,0);
\coordinate (r4) at (10, 0);
\draw[red, dashed]  (r3)--(r4);
%\node[anchor=north west ] at (r4) { %\color{red}$y_2=\bar a_2$};

\node[anchor=north west ] at (1,7) { \color{red}$Q$};

 \end{scope}


==> matching_distance/figures/xPushUpConvexHullExample2.tex <==
\begin{scope}[scale =0.5]


% \coordinate (oo) at (0,0);
 %\coordinate (ox) at (10,0); 
 %\coordinate (oy) at (0, 10); 

 %points u,v,w,x
 \coordinate (u) at (1,2);
 \coordinate (w) at ($(u)+ (5,4)$); 
 \coordinate (v) at (4,0);
 \coordinate (a) at (6,0);
 \coordinate (x) at (9,0.5);
  \coordinate (x') at (4,-2);

 \draw[fill=yellow!10] (w) -- (v) -- (a) -- cycle;
 
%draw points
\draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v=z_l$};
 % \draw[blue, fill=blue] (x) circle (5pt);
 %\node[anchor=north] at (x) { $x$};
  % \draw[blue, fill=blue] (x') circle (5pt);
 %\node[anchor=north] at (x') { $x'$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w=z_r$};
   \draw[red, fill=red] (a) circle (5pt);
  \node[anchor=south] at (a) { $\bar a$};

 %convex hull 
 \draw[fill=red!10] (u) -- (v) -- (w) -- cycle;

%rotation point

%\coordinate (r) at (7.5, 0.25);
 % \draw[red, fill=red] (r) circle (5pt);

%lines
%verical
%\coordinate (l1) at (7.5,-3);
%\coordinate (l2) at (7.5, 10);
%\draw[orange, thick]  (l1)--(l2);
%\node[anchor=north west ] at (l2) { \color{orange}$L$};

%horizontal
%\coordinate (l3) at (0,-1);
%\coordinate (l4) at (10, -1);
%\draw[orange, thick]  (l3)--(l4);
%\node[anchor=north west ] at (l4) { \color{orange}$L'$};

%regions

\coordinate (r1) at (6,-3);
\coordinate (r2) at (6, 10);
\draw[red, dashed]  (r1)--(r2);
%\node[anchor=north west ] at (r2) { %\color{red}$y_1=\bar a_1$};

\coordinate (r3) at (0,0);
\coordinate (r4) at (10, 0);
\draw[red, dashed]  (r3)--(r4);
%\node[anchor=north west ] at (r4) { %\color{red}$y_2=\bar a_2$};
\node[anchor=north west ] at (1,7) { \color{red}$Q$};
 \end{scope}


==> matching_distance/figures/xPushUpConvexHullNonExample.tex <==
\begin{scope}[scale =0.5]


% \coordinate (oo) at (0,0);
 %\coordinate (ox) at (10,0); 
 %\coordinate (oy) at (0, 10); 

 %points u,v,w,x
 \coordinate (u) at (1,2);
 \coordinate (w) at ($(u)+ (4,4)$); 
 \coordinate (v) at (6,0);
 \coordinate (x) at (2,0.5);

%draw points
\draw[blue, fill=blue] (u) circle (5pt);
  \node[anchor=south] at (u) { $u$};
   \draw[blue, fill=blue] (v) circle (5pt);
  \node[anchor=north] at (v) { $v$};
  \draw[blue, fill=blue] (x) circle (5pt);
 \node[anchor=north] at (x) { $x$};
 \draw[blue, fill=blue] (w) circle (5pt);
  \node[anchor=south] at (w) { $w$};

 %convex hull 
 \draw[fill=red!10] (u) -- (v) -- (w) -- cycle;


 
 \end{scope}

